A Model of Enclosures: Coordination, Conflict, and Efficiency in the Transformation of Land Property Rights

Economists, historians, and social scientists have long debated how open-access areas, frontier regions, and customary landholding regimes came to be enclosed or otherwise transformed into private property. This paper analyzes decentralized enclosure processes using the theory of aggregative games, examining how population density, enclosure costs, potential productivity gains, and the broader physical, institutional, and policy environment jointly determine the property regime. Changes to any of these factors can lead to smooth or abrupt changes in equilibria that can result in inefficiently high, inefficiently low, or efficient levels of enclosure and associated technological transformation. Inefficient outcomes generally fall short of second-best. While policies to strengthen customary governance or compensate displaced stakeholders can realign incentives, addressing one market failure while neglecting others can worsen outcomes. Our analysis provides a unified framework for evaluating mechanisms emphasized in Neoclassical, Neo-institutional, and Marxian interpretations of historical enclosure processes and contemporary land formalization policies.

==> litreview.tex <==
Neoclassical economics highlights the crucial role of secure and exclusive private property rights for efficient resource allocation, but largely ignores the practical costs and political complexities of establishing and enforcing such rights. As Abba Lerner wryly observed, ``Economics has gained the title Queen of the Social Sciences by choosing solved political problems as its domain'' \citep[p.259]{lerner1972}.  \citet{weitzman1974} provides a concise elegant illustration, demonstrating that labor will continue to enter open-access land areas until the average product captured equals the opportunity cost of labor, which would be determined by the marginal product on privately owned land. This results in the tragedy of the commons, with inefficiently high application of labor in unenclosed, free-access areas.  Privatization is shown to eliminate the misallocation, but the private property alternative is exogenously and costlessly imposed, and not a result of the decentralized, strategic choices of individual actors.

Recent macro-development papers work within a similar neoclassical framework, but extend the critique of open-access regimes to encompass a broader class customary property regimes. These studies claim that the misallocation inherent in these arrangements can account for a very large portion of measured TFP differences across countries \citep[see e.g.][]{lagakos2013,chen2017a, chen2023, gottlieb2019}. Similar to \citet{weitzman1974}, they focus only on exogenously driven transitions from equilibria with misallocation due to non-exclusive land ownership\footnote{Or, equivalently, a traditional land sector heavily distorted by implied taxes or other distortions.} to an efficient competitive equilibrium with costlessly enforced exclusive private ownership.  They do not address why such customary land property regimes were adopted or why they have persisted and coexisted with private property regimes for so long. While they provide rich macro-economic descriptions of several important general equilibrium implications of a transition away from a mixed property regime, they also typically evade the distributional consequences of privatization by invoking the familiar assumption of lump-sum transfer mechanisms to redistribute the ensuing rents.

New Institutionalist, Austrian, and Marxian economists and other social scientists have offered richer analytical narratives to describe the origin and transformation of land property rights regimes, in theory and in historical practice. A comprehensive review of this immense literature is far beyond the scope of this paper\footnote{An eclectic but very incomplete list of opinionated surveys and books of mostly economic writing on the topic might include \citet{binswanger1995, baland1996, besley2010, ostrom1990, libecap1993, anderson2004, bardhan1989, byres1996, murtazashvili2016a,desoto2000, otsuka2014}}.  One recurring theme, though interpretations vary considerably, is that the cost of establishing and enforcing exclusive property rights often exceed the costs in environments where population density is low, where there may be limited possibilities for trade or technological upgrading, and where state capacity is weak.  Analyses differ greatly, however, on how changes in these or other factors might induce institutional shifts, and through what mechanisms.  To compare these analyses, it is useful to highlight four key dimensions: (1) whether change is primarily evolutionary and negotiated, or conflict-driven and punctuated; (2) whether regimes tend toward efficiency or if inefficient ones can arise and persist; (3) whether change exacerbates or mitigates inequality; and (4) the extent to which regimes emerge organically from decentralized processes or are imposed from above.

The work of many Austrian economists \citep[e.g.][]{murtazashvili2016a}, early New Institutionalists including \citet{alchian1973,demsetz1967, north1973}, along with that of \citet{boserup1965} and \citet{ostrom1990} among others, emphasizes the evolutionary adaptation of resource use and property rights to local circumstances, achieved in part through negotiated settlements and individual entrepreneurship.  A common thread in these perspectives is the general presumption that such adaptations emerge organically and tend towards efficiency, though acknowledging that adaptation takes time and effort and may be disrupted, particularly by outside impositions such as state interventions or rapid changes in technology or market access.

Later new institutionalists including \citet{north1990}  and \citet{acemoglu2005} place more emphasis on power relations, distributional conflicts, and coordination failures in shaping institutional change. While sharing a broadly evolutionary perspective, they argue that coordination failures and other transaction costs often stand in the way of institutional change and that elites often use their power to maintain institutions that serve their interests, even at the cost of societal inefficiency.  Many traditional justifications for state intervention in land registration and titling, or land reform more generally, have been based on the view that inefficient institutions may persist due to coordination failure or the resistance of powerful elites, or `backward peasants'.  Many of these interventions, dating back to Lockean justifications for private property using the language of 'improvements', often overlook existing governance systems or declare them to be inefficient to justify takings or reform in the name of promised increased productivity and investment from more exclusive ownership (Greer, 2018). Whether such interventions, often imposed from above (dimension 4), actually delivered such improvements or mainly served as an excuse for expropriations by more powerful actors (dimension 3) remains a subject of considerable debate.


, arguing that elites may use their power to design institutions that serve their interests, even at the cost of societal inefficiency, potentially leading to persistent inefficient institutions.  In many ways Many traditional justifications for state intervention in land registration and titling or land reform more generally have been based on the view that inefficient institutions may persist, due to coordination failure, or the resistance of powerful elites. Many of these interventions, dating back to Lockean justifications for private property using the language of `improvements', often overlook existing governance systems or declare them to be inefficient, to justify takings or reform in the name of promised increased productivity and investment from more exclusive ownership \citep{greer2018}. Whether such interventions actually delivered such improvements, or mainly served as an excuse for expropriations by more powerful actors 

"Political Marxists" like Robert Brenner \citeyear{brenner1976} and Ellen Wood \citeyear{wood2002} offer a yet more conflict-driven perspective, emphasizing shifts in the balance of class power. They argue that European customary property regimes, while granting peasants possession rights, were inherently inefficient and constrained by feudal legacies, making them unable to adapt. In their view, the transition to capitalism, beginning in England, required a shift in class power that enabled landlords to expropriate the peasantry via enclosures and other means, creating a landless, wage-dependent workforce. This, in turn, fostered the conditions for capitalist imperatives —the drive for continuous productivity increases— to emerge and drove labor release and structural transformation. While this perspective might seem to contrast with more benign interpretations of the state-led efforts to promote the emergence of private property rights and markets, \cite[][p.4]{allen1992} points out that, similar to the neoclassical analyses mentioned above, they share the implied assumption that existing customary property regimes backward and inefficient, and that state-facilitated land titling programs were necessary to overcome coordination failures and other forms of resistance to their removal, that this is what then spurred agricultural productivity growth, and that the increase in inequality that followed was a necessary, albeit perhaps regrettable, consequence of this progress. 

Allen contests the view. Similar to Platteau similarly skeptical

played out in developing countries.

It may seem diffic

Formal models have explored the emergence of private land ownership and its distributional consequences. \citet{weitzman1974} compared free access with private ownership, while \citet{demeza1992} analyzed privately initiated enclosure processes, highlighting the possibility of inefficient equilibria. \citet{cohen1975} examined enclosures from a Marxian perspective, emphasizing potential for increased inequality.


Our model, building on \citet{demsetz1967} and \citet{boserup1965}, captures this complexity, allowing us to analyze efficiency, distributional concerns, and policy implications. We extend the model to incorporate customary tenure regimes with varying degrees of regulation, as emphasized by \citet{ostrom1990} and \citet{platteau1996}. This framework helps explain the mixed success of land formalization programs in developing countries (e.g., \citet{aldenwily2018, platteau1996, desoto2000, deininger2003, lawry2017}). We also explore further extensions, including the relationship between enclosures, labor release, and structural transformation (e.g., \citet{allen1992, crafts2004, matsuyama2008}).



\section{OLD:}


As Abba Lerner wryly explained, ``Economics has gained the title Queen of the Social Sciences by choosing solved political problems as its domain'' \citep[p.259]{lerner1972}. Little in the neo-classical toolkit explains how property rights are upheld or transformed and analyses offer mainly stark and simplified contrasts between private property and alternative property regimes. \citet{weitzman1974} offers a canonical and concise neo-classical framing of the distinction between private property and free- or open-access property regimes. 

New institutionalist and Marxian economists do advance analytical narratives of the endogenous emergence and transformation of property regimes, but they emphasize different and often competing mechanisms and provide little formal modeling. One objective of this paper is to offer an encompassing framework capable of nesting and giving new interpretation to several of these competing interpretations.

One prevalent new-institutionalist narrative is that in regions characterized by low population density and limited market activity, the costs associated with establishing and enforcing exclusive, individualized property rights to land often outweigh the benefits. In such contexts, access rights are typically established through possession and use, and membership in the community with territorial control. Over time, locally adapted informal norms and social pressure, often exerted within existing hierarchical structures, emerge to manage resources with varying degrees of effectiveness \citep{alchian1973, ostrom1990, anderson2004}.

As population density rises further and/or new technological and market opportunities emerge, externalities and conflicts increase. The benefits to establishing more exclusive forms of control over specific plots to mitigate disputes, internalize externalities, or capture new rents and opportunities then become more apparent, to existing users but often also to powerful outsiders as well \citep{boserup1965, ensminger1996}. Whether this leads to institutional and technological change that efficiently adapts to the new challenges and opportunities, or not, and for the benefit of whom, remains the subject of much historical and theoretical research and debate. 

One strand of the literature, often referred to as the Property Rights paradigm, associated with \citet{demsetz1967, alchian1973} and the early Douglas North \citeyearpar{north1973}, emphasizes the possibilities of induced adaptive transformation via evolutionary processes. Although some emphasize the potential for Coasian bargains \citeyearpar{coase1960} to yield transaction cost-minimizing solutions \citep{anderson2004}, others have employed this framework to advocate for state intervention in land titling, citing perceived inefficiencies of communal land ownership and its resistance to transformation.

This view of customary tenure as inherently inefficient has deep intellectual roots in Western political thought. John Locke's theory of property, which heavily influenced colonial doctrine, argued that private property rights arise when individuals mix their labor with land to create "improvements," implicitly delegitimizing indigenous forms of land use that did not match European agricultural practices. This perspective often incorrectly equates unenclosed land with open-access, invoking Hardin's "tragedy of the commons" \citep{hardin68} while ignoring existing systems of collective governance. Recent macro-development literature continues this tradition, measuring potential efficiency gains from replacing customary systems with private property \citep{chen2017a, chen2023}. However, these analyses take the property regime and its transformation to be exogenous and do not consider the costs of establishing and maintaining a more efficient private property system. The distributional consequences for existing customary rights holders are largely swept aside by assuming costless redistributive transfers or Coasian bargains.

\citet{platteau1996} describes this collection of views as part of the Evolutionary Theory of Land Rights (ETLR), because even those that decry the failures of customary systems tell a narrative of endogenous evolutionary change by arguing that interventions by government or policy entrepreneurs respond to endogenous political 'demands' for change.

The transformation of property rights based on possession and use to more exclusive private property rights, especially when done via state-sacntioned land formalization programs, has remained contentious in both theory and historical practice.  One prevalent view, traceable from

A different interpretation of institutional change is provided by scholars that emphasize the role of politics and power. Douglass North in his later writings, along with more recent interpreters including Acemoglu and Robinson, argue that institutional change is shaped by elite political and economic interests. This perspective suggests that private and social interests may diverge, leading to the emergence and persistence of inefficient property arrangements and sometimes sudden shifts in institutional arrangements rather than smooth transformation \citep{north1990, acemoglu2000}. Political Marxists like Robert Brenner place even greater emphasis on the role of class struggle and state coercion. Brenner argued that shifts in the balance of class forces are what enabled English landlords to employ enclosures and other mechanisms to sweep away customary property regimes and dispossess peasants to transform them into wage-dependent laborers - processes that they see as essential to modern capitalist development \citep{brenner1976, wood2002}.


A more nuanced perspective recognizes that while customary regimes may generate inefficiencies through excess entry and foregone outside opportunities, transition costs and distributional consequences matter. \citet{ostrom1990} and \citet{platteau1996} document how customary systems often manage to effectively manage resources through complex combinations of individual and collective rights. Unlike idealized private property with absolute rights to exclude and transfer, actual customary regimes typically involve \textit{de facto} possession rights structured within community rules and hierarchical relationships \citep{ribot2003, sjaastad1997}.

%% Need to revise remaining paragraphs
The establishment of private ownership can promote efficiency and investment benefits, but these benefits must be weighed against the possibly higher costs of enforcement associated with the operation of more formal system of private property. Property regime transitions are inherently political and hence, depending on design, could produce significant distributional changes and social tensions.  Whether such changes to circumstances and individual incentives will precipitate successful institutional or technological changes or not, and whether any transition is gradual and negotiated or sudden and imposed, generally depends on historical context, and the nature of the strategic interaction processes. 

Considerations of this sort dominated important historical debates surrounding property rights transitions such as those associated with the Enclosure Movements in England, the establishment of property rights on the frontiers of new colonies or newly forming nations states, and in contemporary efforts to recognize, register and formalize new or existing plot owners in rural, peri-urban, and urban land settlements in developing countries today.

It has commonly been assumed that land that is not exclusively owned will become subject to the so-called ``tragedy of the commons'' \citep{hardin68}, where individuals are led to overuse and deplete commonly owned resources. Private and exclusive ownership, as \citet{demsetz1967, alchian1973} famously suggested, promotes efficient use of land by providing individuals with incentives to maximize the value of their property and, consequently, private ownership should emerge when these benefits exceed the costs of delineating property rights. 

The literature highlights several potential advantages of enclosure and private ownership.  By providing secure and exclusive rights, private property can incentivize efficient resource allocation, release labor resources that would have gone to establishing possession, promote investment in technology and land improvements, and facilitate market development \citep[e.g.][]{richardcornes1996, eggertsson1990, besley2010}. \citet{boserup1965}, who argued that increasing population pressure often drives agricultural intensification and the adoption of more exclusive forms of private land ownership. 

However, as \citet{coase1960} emphasized, the benefits of establishing any new institution must always be weighed against its costs \citep[see also][]{alchian1973, north1973}. The social benefits of more exclusive ownership may outweigh the social costs of enforcement in some environments, but not others. A pastoral society with an abundance of fertile land may find little value in fences. Even in modern societies, fencing off the seas, open spaces, and many other resources may be impractical and prohibitively expensive. At a more practical level, even where land formalization programs might be initiated by policy design, enclosure processes are ultimately decentralized affairs. The decision to enclose a particular plot, or not, will be determined by the equilibrium actions of would-be claimants who consider local circumstances and the strategic decisions of others in balancing expected benefits against the costs of pressing for more exclusive forms of ownership. Whatever the source of the benefits of private ownership, the costs of delineating property rights include surveying, fencing, legal disputes, and enforcement mechanisms. \citet{baker2003, baker2008} and \citet{hafer2006} are among those who focus more on the structure of these enforcement costs and how they interact with strategic concerns. 

There has been much formal work on the emergence of private land ownership, and this formal modeling has led to a more thorough assessment of the relationship between enclosure and the distribution of income. In an early work, \citet{weitzman1974} compared free access with private ownership, highlighting the distribution of income to labor, concluding that variable factors were always better off under free access, despite any use inefficiency resulting from common property. Several more recent textbook-level treatments exist \citep[see e.g.][]{baland1996, richardcornes1996, dasgupta1980}, which address inefficiency issues in more detail. \citet{demeza1992} offered an important addition by emphasizing the relatively understudied question of privately initiated and privately costly enclosure processes. Employing well-chosen examples from a reduced-form model, they demonstrated a range of possible equilibrium outcomes in the privatization of a pure open-access resource, including inefficient equilibria with either too much or too little enclosure, and multiple equilibria.  

The transition from common property to private ownership often results in significant distributional changes, as emphasized by \citet{brenner1976}, and formally analyzed by \citet{cohen1975}, who consider enclosures from an explicitly Marxian perspective, emphasizing the displacement of small farmers and the concentration of land in the hands of a few wealthy individuals. They found that the enclosure process can exacerbate income inequality and create social tensions. 

There has also been much pushback on the dichotomous nature of these comparisons, in which enclosure and private ownership is assumed to be naturally more efficient than alternative ownership structures. \citet{ostrom1990} and \citet{platteau1996} provide empirical evidence of the successful collective management of common-pool resources, highlighting the role of community norms and local governance structures. Moreover, actual property regimes tend to have a hybrid form, making comparison with the commons more difficult. Unlike modern private property, where owners theoretically hold \textit{de jure} absolute rights to exclude and transfer, these systems often rely on \textit{de facto} maintained possession and use within rule-structured communities and/or hierarchical relationships. Transfers, especially to outsiders, are often limited \citep{ribot2003, sjaastad1997,hoffmann2015}. Resources that appear to be open-access are, in reality, collectively managed and regulated, often quite strictly, through emergent formal and informal laws, rules, and customs. Under many customary forms of tenure, individual families often also hold rights to specific plots that may even become heritable or subject to rental or sale, particularly when traded is limited to other members of the community.  Likewise, would-be enclosers often already hold claims under prevailing informal or customary property regimes and encounter resistance and/or will be forced to offer compensation to users whose competing claims might be diminished or extinguished by their enclosing activities. The British Parliamentary Enclosure Acts, for example, required negotiated settlements and various forms of compensation to displaced commoners and other stakeholders \citep{mccloskey2015, heldring2022}. 

Indeed, there is a large, detailed literature on the historical experience of enclosure, much focusing on the millennia-long process of enclosure in England. This literature has provided direct empirical evidence on the enclosure experience and sheds much light on both efficiency and distributional consequences of enclosure relative to institutions that existed prior to enclosure. \citet{allen1992} and \citet{heldring2022} highlight the economic benefits of enclosures, including increased agricultural productivity and economic growth. They also acknowledge the social costs of enclosure, such as those arising from the displacement of small farmers and changes in rural labor markets. Political Marxists such as \citet{brenner1976} and \citet{wood2002} have argued that enclosures formed part of a larger process of `primitive accumulation' that took place with consequential effects in Britain, particularly from the 16th to the 18th centuries. They argue that shifts in political power allowed English landlords to erode peasant rights of possession and displace laborers in ways that ultimately resulted in a largely landless low-wage, market-dependent rural proletariat, which they argue was essential for the creation of capitalist imperatives and accumulation. It has also been argued that enclosures can increase labor demand and wages and produce net pecuniary benefits even as households lose or give up possession, more consistent with non-Marxist interpretations \citet{chambers1966, whittle2013}.  

Recent experience with enclosure, or more broadly, the privatization of land ownership as it relates to economic development, has provided new challenges, as a goal of policy is often to balance efficiency and equity. \citet{deininger2003} discuss land policies for growth and poverty reduction, emphasizing the need for secure land rights to encourage investment and economic development. \citet{binswanger1995} go a step further and explore the impact of power, distortions, and reforms on agricultural land relations, highlighting the challenges of implementing equitable land policies. \citet{aldenwily2018} examines the resurgence of collective land ownership in the 21st century, noting that collective land rights can help address inequality issues and provide communities with a sense of security and identity. This literature poses some mysteries. In some environments, land formalization programs have failed to generate sufficient private take-up demand, as people prefer to retain or rely on customary property regimes \citep[e.g.][]{ali2019, jacoby2007}. In other situations, similar programs have created rent-seeking opportunities that led to abuse or sparked costly and difficult-to-control property races \citep{anderson1990,leeson2018a}.  

Our model is built on the basic forces delineated by \citet{demsetz1967} and \citet{boserup1965} so that it can capture the wealth of possible outcomes while also providing insight into efficiency and distributional concerns. This allows us to assess policy in Section \ref{policy_both}, where we argue that land policy is subject to the theory of the second best, in that policies designed to address one market failure without taking into account other market failures can lead to worse outcomes. For example, policies to strengthen customary land governance and regulation to correct labor misallocation, that do not at the same time also establish compensation schedules for those who might be displaced by enclosures, can inadvertently increase the likelihood of costly property scrambles. However, policies that simply increase mandated compensation to the displaced without also strengthening governance and regulation within customary areas can inadvertently increase the likelihood of coordination failures that delay or otherwise impede efficient enclosure to facilitate technological transformation. Our extended model, introduced later in the paper in section \ref{extended_model}, extends the basic model to one in which we can assess `customary tenure' regimes that are regulated to varying degrees by access fees or customary rents, the importance of which has been emphasized by \citet{ostrom1990} and \citet{platteau1996}, for example. Collectively, these insights from our theoretical model help to understand why, despite waves of enabling legislation and several decades of attempted land formalization programs in developing countries, many of these programs have been delayed or scuttled due to low acceptance and / or concerns surrounding their distributional and efficiency consequences \citep{aldenwily2018, platteau1996, desoto2000, deininger2003, lawry2017}. We also pursue some other extensions of the model (in Section \ref{sec-encompass}) that shed further light on policy, efficiency, and distribution, including the a discussion of the debated relationships between enclosures, labor release, structural transformation, and the growth of manufacturing \citep{allen1992, crafts2004, matsuyama2008}. 
